Object-based (yet Class-agnostic) Video Domain Adaptation

Existing video-based action recognition systems typically require dense annotation and struggle in environments when there is significant distribution shift relative to the training data. Current methods for video domain adaptation typically fine-tune the model using fully annotated data on a subset of target domain data or align the representation of the two domains using bootstrapping or adversarial learning. Inspired by the pivotal role of objects in recent supervised object-centric action recognition models, we present Object-based (yet Class-agnostic) Video Domain Adaptation (ODAPT), a simple yet effective framework for adapting the existing action recognition systems to new domains by utilizing a sparse set of frames with class-agnostic object annotations in a target domain. Our model achieves a +6.5 increase when adapting across kitchens in Epic-Kitchens and a +3.1 increase adapting between Epic-Kitchens and the EGTEA dataset. ODAPT is a general framework that can also be combined with previous unsupervised methods, offering a +5.0 boost when combined with the self-supervised multi-modal method MMSADA and a +1.7 boost when added to the adversarial-based method TA$^3$N on Epic-Kitchens.

==> sec/intro_backup.tex <==
\def\FigTeaser#1{
\begin{figure}[#1]
\begin{center}
\includegraphics[width=\linewidth]{Figure/teaser.pdf}
\end{center}
\vspace{-1.2em}
\caption{(a) Fully-supervised approaches use video clips with action labels to fine-tune the action recognizer trained in the source domain. (b) The state-of-the-art self-supervised based on adversarial learning try to align the representation between source and target from both spatial and temporal aspects. (c) Our proposed \Ours keeps the action recognizer frozen while only adapting the object information to the target domain.}
\label{fig:teaser}
\vspace{-1em}
\end{figure}
}

\FigTeaser{!t}



\section{Introduction}
\label{sec:intro}

\noindent \dantong{the goal of this paper}

In practical scenarios, such as customizing an action recognition model for a specific smart home, performance degradation is always observed when the model is exposed to a previously unknown environment. The disparity between the old and the new environment exacerbates this issue. Addressing this challenge is crucial as it significantly affects functionality. A commonly employed strategy is to frame this as a domain adaptation problem, with the goal to bridge the gap between the source and target domains.

% Consider a realistic and practical problem: we wish to adapt an existing action recognition model to a new environment (\eg, adapt a smart home assistant to a particular home), the performance decreases because the home assistant never ``see'' this new home. This phenonmenon will be worse with the crease of the difference of the two environments, making it significant to solve it. A common solution is to treat this as domain adaptation problem.




\noindent \dantong{Related works and limitations}

Supervised domain adaptation approaches assumes the availability of annotated data from the target domain, a condition not always met in real-world applications. These methods necessitate extensive labeled video data from the new environment to fine-tune the action recognition model, as illustrated in ~\cref{fig:teaser} (a). However, the resource-intensive nature of data acquisition, processing, and labeling, alongside the need for substantial model fine-tuning, renders this approach impractical in many cases. In scenarios where acquiring labeled data is exceedingly expensive or infeasible, unsupervised domain adaptation methods become relevant. These methods, including adversarial and contrastive learning strategies referenced in\cite{adda, dann, ta3n, choi2020shuffle, sahoo2021contrast, munro2020multi}, aim to align the representations of the source and target domain in both temporal and spatial dimensions, as depicted in~\cref{fig:teaser} (b). Despite their utility, these unsupervised methods often entail extended adaptation periods and their performance significantly lags behind that of fully-supervised counterparts, particularly when there is a pronounced divergence between the source and target domains.


% Supervised approaches assume we have access to the target domain, which is not always true in practical, they require fully-annotated videos in the new environment to fine-tune the action recognition model (~\cref{fig:teaser} (a)). However, this approach is super costly both in terms of data collection, processing and labeling, and the required fine-tuning of the action recognition model. When labels in the new environment are prohibitively costly or impossible to obtain, unsupervised domain adaptation approaches can be employed, utilizing adversarial and/or contrastive learning \cite{adda, dann, ta3n, choi2020shuffle, sahoo2021contrast, munro2020multi}  which align the representations between the source and target domain in temporal and/or spatial aspects (\cref{fig:teaser} (b)). However, these approaches suffer from long adaptation time and still the performance is much far from the upper bound (fully-supervised strategies), especially when the target domain is largely diverged from the source domain.

\noindent \dantong{Our insight}

In this paper, we present Object-driven Video Domain Adaptation (abbreviated as \Ours), which dramatically reduces the need for annotated data to less than 1\% compared to traditional supervised methods for video domain adaptation. The inspiration for \Ours comes from several pioneering object-centric action recognition studies~\cite{arnab2021unified,svit2022,herzig2022orvit,Wang_videogcnECCV2018}, which have shown that the explicit modeling of objects and hands significantly enhances the recognition of complex actions, such as human-object interactions. These studies typically employ integrated object detectors to gather object and hand information to bolster the primary task. \Ours leverages this concept by utilizing an extremely sparse set of frames from the target domain, annotated with object and hand labels, to adapt only the object-centric information. \Ours streamlines the domain adaptation process by focusing on module rich in object-centric imformation rather than adapting the entire action recognition system.

% We propose Object-driven Video Domain Adaptation (\Ours for short), a general framework that utilized less than $1\%$ (\vs supervised methods) for the video domain adaptation. \Ours is inspired by several recent object-centric action recognition works~\cite{arnab2021unified,svit2022,herzig2022orvit,Wang_videogcnECCV2018}. These work demonstrates that recognizing complex actions (such as human-object interactions) strongly benefits from explicitly modeling objects and/or hands, they utilize integrated object detectors to obtain object and hand information to assist the main task. \Ours proposes to take advantages of the object-centric information to assist the domain adaptation. Specifically, \Ours utilizes an extremely sparse set of frames in the target domain with labeled hands and objects to only adapt these object-centric information instead of adapt the whole action recognizer.


\noindent \dantong{Our approach}

With the hypothesis that enhanced object information in an unseen environment contributes to narrowing the domain gap, \Ours demonstrates its simplicity and efficacy as depicted in~\cref{fig:teaser} (c). The method begins with an existing structured action recognizer, which includes an auxiliary object-centric module, trained on the source domain. \Ours solely adapts this auxiliary module through fine-tuning while keeping the rest frozen, thus significantly reducing adaptation time in comparison to both supervised full model adaptation and unsupervised feature alignment. \Ours requires a sparse set of frame-level labels (less than 1\% of the frames within the target domain relative to the fully-annotated video dataset). Moreover, these frames are ``object-sparse'': we only focus on the bounding boxes for hands and the objects they interact with. Obtaining such data is largely facilitated by the utilization of SAM~\cite{kirillov2023segment}.

% With the hypothesis that better object information in the unseen environment can help close the domain gap, \Ours is simple yet effective as shown in~\cref{fig:teaser} (c): given an existed structured (with auxiliary object-centric module)  action recognizer trained in the source domain, \Ours only adapts the auxiliary module by fine-tuning and leaves the rest as frozen, making the adaptation time much shorter (\vs supervised full model adapting and unsupervised feature alignment). \Ours uses a super sparse set of frame-level (1\% frames in the target domain \vs the fully-annotated number of videos) labels in the adapting. Additional, these 1\% frames are object-sparse, for we only need bounding boxes for hands and objects interacted with hands, which is easy to get with favor of SAM~\cite{kirillov2023segment}.





\noindent \dantong{Our Results}

We construct a challenging scenario to implement \Ours, using ego-centric cooking datasets Epic-kitchens~\cite{Damen2018EPICKITCHENS,damen2020epic} and EGTEA Gaze+ videos~\cite{li2018eye} , that both capture egocentric cooking actions. They are distinct in terms of the used hardware, recording setup, and annotation protocols, thus presenting a substantive domain gap. Our results show that adapting object-centric information makes a difference in mitigating the domain gap between the source and target domain. For ViT-based structured action recognition models (ORViT~\cite{herzig2022orvit} is used in our experiment),  \Ours achieves +6.5 performance on Epic-kitchens, +3.1 on EGTEA. For non-structured action recognition models, there are some previous domain adaptation methods~\cite{ta3n, munro2020multi, sahoo2021contrast}, \Ours brings further boost when adapted to these methods. Specifically, TA$^3$N-\Ours achieves +1.7 increase than TA$^3$N~\cite{ta3n}, MMSADA-\Ours achieves +5.0 increase than MMSADA~\cite{munro2020multi}, CoMix-\Ours achieves +1.7 increase than CoMix~\cite{sahoo2021contrast} on Epic-Kitchens~\cite{damen2020epic}.

\noindent \dantong{Contribution}

In summary, the principal contribution is the introduction of \Ours. \Ours is distinguished by its simplicity and efficacy, demonstrating considerable improvements in video domain adaptation with the utilization of less than 1\% of the labeled data required by traditional methods. Furthermore, \Ours's versatile design allows it to be applied effectively across a variety of action recognition models, regardless of their structural differences.

% In summary, the main contribution of this work is we present \Ours, a simple but effective frame work. performing well in video domain adaptation while only uses less than 1\% labels. \Ours is general framework that works for action recognizers with different structures. 



